Towards Robust Classification Model by Counterfactual and Invariant Data Generation

Despite the success of machine learning applications in science, industry, and society in general, many approaches are known to be non-robust, often relying on spurious correlations to make predictions. Spuriousness occurs when some features correlate with labels but are not causal; relying on such features prevents models from generalizing to unseen environments where such correlations break. In this work, we focus on image classification and propose two data generation processes to reduce spuriousness. Given human annotations of the subset of the features responsible (causal) for the labels (e.g. bounding boxes), we modify this causal set to generate a surrogate image that no longer has the same label (i.e. a counterfactual image). We also alter non-causal features to generate images still recognized as the original labels, which helps to learn a model invariant to these features. In several challenging datasets, our data generations outperform state-of-the-art methods in accuracy when spurious correlations break, and increase the saliency focus on causal features providing better explanations.

==> junk_from_bib <==
% @String(PAMI  = {IEEE TPAMI})
% @String(IJCV  = {IJCV})
% @String(CVPR  = {CVPR})
% @String(ICCV  = {ICCV})
% @String(ECCV  = {ECCV})
% @String(NIPS  = {NeurIPS})
% @String(ICPR  = {ICPR})
% @String(BMVC  =	{BMVC})
% @String(TOG   = {ACM TOG})
% @String(TIP   = {IEEE TIP})
% @String(TVCG  = {IEEE TVCG})
% @String(TCSVT = {IEEE TCSVT})
% @String(TMM   =	{IEEE TMM})
% @String(ACMMM = {ACM MM})
% @String(ICME  =	{ICME})
% @String(ICASSP=	{ICASSP})
% @String(ICIP  = {ICIP})
% @String(ACCV  = {ACCV})
% @String(ICLR  = {ICLR})
% @String(IJCAI = {IJCAI})
% @String(PR = {PR})
% @String(AAAI = {AAAI})
% @String(CVPRW= {CVPRW})
% @String(CSVT = {IEEE TCSVT})



% @String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
% @String(IJCV = {Int. J. Comput. Vis.})
% @String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
% @String(ICCV= {Int. Conf. Comput. Vis.})
% @String(ECCV= {Eur. Conf. Comput. Vis.})
% @String(NIPS= {Adv. Neural Inform. Process. Syst.})
% @String(ICPR = {Int. Conf. Pattern Recog.})
% @String(BMVC= {Brit. Mach. Vis. Conf.})
% @String(TOG= {ACM Trans. Graph.})
% @String(TIP  = {IEEE Trans. Image Process.})
% @String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
% @String(TMM  = {IEEE Trans. Multimedia})
% @String(ACMMM= {ACM Int. Conf. Multimedia})
% @String(ICME = {Int. Conf. Multimedia and Expo})
% @String(ICASSP=	{ICASSP})
% @String(ICIP = {IEEE Int. Conf. Image Process.})
% @String(ACCV  = {ACCV})
% @String(ICLR = {Int. Conf. Learn. Represent.})
% @String(IJCAI = {IJCAI})
% @String(PR   = {Pattern Recognition})
% @String(AAAI = {AAAI})
% @String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
% @String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

% @String(SPL	= {IEEE Sign. Process. Letters})
% @String(VR   = {Vis. Res.})
% @String(JOV	 = {J. Vis.})
% @String(TVC  = {The Vis. Comput.})
% @String(JCST  = {J. Comput. Sci. Tech.})
% @String(CGF  = {Comput. Graph. Forum})
% @String(CVM = {Computational Visual Media})



% @misc{Authors14,
%  author = {FirstName LastName},
%  title = {The frobnicatable foo filter},
%  note = {Face and Gesture  submission ID 324. Supplied as additional material {\tt fg324.pdf}},
%  year = 2014
% }

% @misc{Authors14b,
%  author = {FirstName LastName},
%  title = {Frobnication tutorial},
%  note = {Supplied as additional material {\tt tr.pdf}},
%  year = 2014
% }

% @article{Alpher02,
% author = {FirstName Alpher},
% title = {Frobnication},
% journal = PAMI,
% volume = 12, 
% number = 1, 
% pages = {234--778}, 
% year = 2002
% }

% @article{Alpher03,
% author = {FirstName Alpher and  FirstName Fotheringham-Smythe},
% title = {Frobnication revisited},
% journal = {Journal of Foo},
% volume = 13, 
% number = 1, 
% pages = {234--778}, 
% year = 2003
% }

% @article{Alpher04,
% author = {FirstName Alpher and FirstName Fotheringham-Smythe and FirstName Gamow},
% title = {Can a machine frobnicate?},
% journal = {Journal of Foo},
% volume = 14, 
% number = 1, 
% pages = {234--778}, 
% year = 2004
% }
